PInKS: Preconditioned Commonsense Inference with Minimal Supervision

Reasoning with preconditions such as "glass can be used for drinking water unless the glass is shattered" remains an open problem for language models. The main challenge lies in the scarcity of preconditions data and the model's lack of support for such reasoning. We present PInKS, Preconditioned Commonsense Inference with WeaK Supervision, an improved model for reasoning with preconditions through minimum supervision. We show, both empirically and theoretically, that PInKS improves the results on benchmarks focused on reasoning with the preconditions of commonsense knowledge (up to 40% Macro-F1 scores). We further investigate PInKS through PAC-Bayesian informativeness analysis, precision measures, and ablation study.

==> Sections/Dummy_Expr_abalation.tex <==
As a final study, we focus on different aspects of \weakcq and evaluate how each step is contributing to the results.
There are three questions we seek to answered.
First, how does each labeling function (LF) is contributing to the extracted preconditions?
%Second, to what extend do the weak supervision data contribute? (addressed in \Cref{subsec:target-tasks})
Second, how much does the precondition-aware masking (\Cref{subsec:modified-mlm}) effect the overall performance of \weakcq.
Here, we try to address these question.


\muhao{ablation is needed for w/ and w/o generative data augmentation on at least one target task. Otherwise, there is no evidence to show that the weak supervision from data augmentation is effective. Missing this evidence is a \textbf{severe} flaw since 3.2 introduced data augmentation as a key technical component, but no justification has been provided for this component.}


\paragraph{Effectiveness of Biased Masking}
For the third question, we focus on \CQ as the target task and compare the results of \weakcq with an alternative setup with no biased masking. 
In the alternative setup, we only use the weak-supervision data that we extract to fine-tune the RoBERTa-Large-MNLI model and compare the results.
Our results show that the \fmac score for zero-shot transfer learning setup drops to $68.4\%$ (from $69.5\%$) without biased masking process. 

\muhao{where is the answer to the first question then? We cannot have an ablation study that studies only one technical component.}

==> Sections/Dummy_Expr_pabi.tex <==
\pabi~\cite{forseeing} proposes a unified PAC-Bayesian motivated informativeness measure that correlates with the improvements provided by the incidental signals to showcase its effectiveness on a target task.
The incidental signal can include an inductive signal, e.g.\ partial/noisy labeled data, or a transductive signal, e.g.\ cross-domain signal in transfer learning.
In this experiment, we go beyond the empirical results and use the \pabi measure to showcase how improvements from \weakcq are theoretically justified.
Here, we use the \pabi score for cross-domain signal assuming the weak supervised data portion of \weakcq (\Cref{subsec:labeling} and \Cref{subsec:augmentation}) as a indirect signal for a given target task.
We use \pabi measurements from two perspective, first, how useful is the weak supervised data portion of \weakcq for
target tasks in comparison with fully-supervised data; and second, how the \recall score affects this usefulness.

\paragraph{Setup}
We carry over the setup on models and tasks from~\Cref{subsec:target-tasks}.
For details on the \pabi itself and the measurement details associated with it, please see~\Cref{sec:details-on-pabi}.


\paragraph{Discussion}
\Cref{tab:pabi-eval} summarizes the \pabi informativeness measure in comparison with other datasets with respect to \CQ~\cite{qasemi2021corequisite} and $\delta$-NLI~\cite{rudinger2020thinking}.
To facilitate the comparison of \pabi scores in \Cref{tab:pabi-eval}, we have also reported the minimum achievable (Zero Rate classifier) and maximum achievable \pabi scores.
To clarify, to compute the maximum achievable \pabi score, we assume the training subset of \CQ and $\delta$-NLI as an indirect signal for the test subset.
Here, we assume that the training subset is in practice the most informative indirect data available.
% Here, the \weakcq is compared with the rest of the datasets when each are considered as incidental signal, for $\delta$-NLI~\cite{rudinger2020thinking} and CoreQuisit~\cite{qasemi2021corequisite} as target tasks.
% As shown here, the theoretical informativeness measures of \weakcq are consistent with the results from \Cref{tab:target-eval}.\qiang{explain the consistency explicitly. At least I'm a little confused here.}

Our results show that although, \weakcq is not the top informative incidental signal on the both target dataset, its \pabi numbers are still significant considering that its the only weak-supervision data which is automatically acquired, while others are acquired based on human annotations.

\begin{table}[ht]
    \small
    \centering
    \setlength\tabcolsep{1pt}
    \begin{tabularx}{\linewidth}{l|cc|X}
         \hline
         & \multicolumn{2}{c|}{\textbf{\pabi on}} &
        \\
            
            \textbf{Indir. Task}
            & \textbf{\CQ}
            & \textbf{$\delta$-NLI}
            & \textbf{Explanation}
        \\
        \toprule
        \weakcq      & 37 & \blpinked{\textit{67}} & - Best on $\delta$-NLI \\ \hline
        $\delta$-NLI & \blpinked{\textit{52}} & \blreded{\textbf{86}} & - Max achievable on $\delta$-NLI \\ &&& - Best on \CQ  \\
        \CQ           & \blreded{\textbf{52}} & 31 & - Max achievable on \\&&&\CQ \\
        ANION        & 34 & 14\\
        ATOMIC       & 21 & 17 \\
        Winoventi    & 36 & 53\\ 
        \hline
        Zero Rate & 26 & 0 & - Baseline\\ 
        \bottomrule
    \end{tabularx}
    \caption{\pabi informativeness measures (x100) of \weakcq and other target tasks w.r.t \CQ and $\delta$-NLI. \blreded{\textbf{Bold}} values represent the maximum achievable \pabi Score by considering train subset as an \emph{indirect} signal for test subset of respective data. The highest \pabi score is selected in \blpinked{\textit{italic}}.\muhao{This caption is confusing: why there is a maximum achievable \pabi Score, then another highest \pabi score?}
    % \muhao{Suggest to remove \CQ and $\delta$-NLI which provide direct supervision to target tasks.}
    % \qiang{the language of PABI is the informativeness of a source data for a target data. Is the ``target data'' in this table actually the source data in PABI? to improve on naming, you can call the first column ``indirect signal''? (we use ``indirect'' and ``incidental'' almost interchangeably in Dan's group, but in publications we try to use ``indirect'' instead of ``incidental'' to avoid confusions.)}
    }
    \label{tab:pabi-eval}
    % \vspace{-1em}
\end{table}

% \begin{table}[ht]
%     \small
%     \centering
%     \begin{tabular}{l|ll}
%         \textbf{Indirect Data}
%             & \textbf{\pabi on \CQ}
%             & \textbf{\pabi on $\delta$-NLI}
%         \\
%         \hline
%         Target Data & 52.3 & 85.5 \\
%         Best Sup. & 52.2 ($\delta$-NLI) & 53.4 (Winoventi) \\
%         \weakcq & 36.6 & 19.1 \\
%         Worst Sup. & 20.9 (ATOMIC) & 13.9 (ANION) \\
%         Zero Rate & 25.5 & 0.0 \\
        
%         % \weakcq      & 36.6 & 19.1 \\
%         % $\delta$-NLI & 52.2 & \textbf{85.5} \\
%         % \CQ           & \textbf{52.3} & 31.3 \\
%         % ANION        & 34.1 & 13.9\\
%         % ATOMIC       & 20.9 & 17.4 \\
%         % Winoventi    & 36.4 & 53.4\\
%         \hline
%     \end{tabular}
%     \caption{\pabi informativeness measures (x100) of \weakcq, compared to the supervised resources w.r.t test subset of \CQ and $\delta$-NLI. Target data is the \pabi considering train subset of the same task as incidental signal and is the maximum achievable.
%     }
%     \label{tab:pabi-eval}
% \end{table}


% \paragraph{Discussion}\qiang{why is this paragraph repeated?}
% \Cref{tab:pabi-eval} summarizes the \pabi informativeness measure.
% Here the \weakcq is compared with the rest of the dataset when considered all as incidental signal, and $\delta$-NLI and \CQ as target tasks.
% As shown here, the theoretical informativeness measures of \weakcq are consistent with the results from \Cref{tab:target-eval} for both target tasks.
% Here although \weakcq is not the top informative incidental signal on the target dataset, its \pabi measures are still significant considering it is the only weak-supervision data.




==> Sections/Dummy_Expr_recall.tex <==
\muhao{This subsection should be merged to 4.2. Discussing Informativeness vs. \Recall should be a part of discussing
Informativeness Measure.
4.2 alone also does not have enough content.}

As mentioned in \Cref{subsec:extracting-action-prec}, each linguistic pattern is assigned a \recall value calculated
from expert annotations on its matches.
Using this \recall value coupled with the \pabi informativeness measure, we can investigate the effect of the
linguistic pattern's \recall on quality of the extracted data.

\paragraph{Setup}
The model setup in this section is the same as the~\Cref{subsec:target-tasks} and~\Cref{subsec:info-vs-recal}.
Here, we create different versions of \weakcq with different levels of \recall threshold (e.g. $0.0$, $0.5$) and
compare their informativeness on \CQ~\cite{qasemi2021corequisite} with \weakcq's (\recall $0.75$) informativeness.
To limit the computation time, we only use $100K$ samples from \weakcq in each threshold value, which is especially
important in lower thresholds due to huge size of extracted patterns with low \recall threshold.


\paragraph{Discussion}
\Cref{tab:recal-eval} summarizes the \pabi informativeness estimation on weak supervision data under three threshold levels of recall on, and compare them with \QT{zero rate} classifier (always predicting major class).
As illustrated, the informativeness show a significant drop in lower recall showcasing the importance of using high recall templates in our weak-supervision task.
For higher thresholds ($0.95$) the data will mostly consist of \emph{allow} patterns, the model drops to near zero rate informativeness baseline.
This susceptibility on pattern recall can be mitigated with having more fine-grained patterns on larger corpora. 
We leave further analysis on recall of patterns to future work.
\muhao{this discussion reads also like a part of 4.2. Indeed this whole subsection should be merged to 4.2.}
% \begin{table}[ht]
%     \small
%     \centering
%     \begin{tabular}{l|l}
%         \textbf{Source Data}
%             & \textbf{\pabi on \CQ}
%         \\
%         \hline
%         Zero Rate             & 26 \\
%         \weakcq-recall-0.00   & 24 \\
%         \weakcq-recall-0.50   & 26 \\
%         \weakcq-recall-0.70   & 37 \\
%         \weakcq-recall-0.95   & 26 \\
%         \hline
%     \end{tabular}
%     \caption{\pabi informativeness measures of \weakcq with different recall thresholds on \CQ.
%     }
%     % \qiang{what about an even higher recall, say 0.8? From this table above, it's obvious that the higher the recall, the higher the informativeness score. Then one may wonder why don't you try an even higher recall -- maybe that informativeness score is even higher?}
%     \label{tab:recal-eval}
% \end{table}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{AssetsRecall-vs-PABI.png}
    \caption{\pabi informativeness measures of \weakcq with different recall thresholds on \CQ.}
    \label{tab:recal-eval}
\end{figure}
